Relation Matters in Sampling: A Scalable Multi-Relational Graph Neural Network for Drug-Drug Interaction Prediction

Sampling is an established technique to scale graph neural networks to large graphs. Current approaches however assume the graphs to be homogeneous in terms of relations and ignore relation types, critically important in biomedical graphs. Multi-relational graphs contain various types of relations that usually come with variable frequency and have different importance for the problem at hand. We propose an approach to modeling the importance of relation types for neighborhood sampling in graph neural networks and show that we can learn the right balance: relation-type probabilities that reflect both frequency and importance. Our experiments on drug-drug interaction prediction show that state-of-the-art graph neural networks profit from relation-dependent sampling in terms of both accuracy and efficiency.

==> paper_ijcai <==
\begin{thebibliography}{}

\bibitem[\protect\citeauthoryear{Bordes \bgroup \em et al.\egroup
  }{2013}]{fb15k}
Antoine Bordes, Nicolas Usunier, Alberto Garcia-Duran, Jason Weston, and Oksana
  Yakhnenko.
\newblock Translating embeddings for modeling multi-relational data.
\newblock In {\em Proc. of NeurIPS}, pages 2787--2795. 2013.

\bibitem[\protect\citeauthoryear{Chen \bgroup \em et al.\egroup
  }{2018a}]{chen2018stochastic}
Jianfei Chen, Jun Zhu, and Le~Song.
\newblock Stochastic training of graph convolutional networks with variance
  reduction.
\newblock In {\em Proc. of ICML}, pages 942--950, 2018.

\bibitem[\protect\citeauthoryear{Chen \bgroup \em et al.\egroup
  }{2018b}]{chen2018fastgcn}
Jie Chen, Tengfei Ma, and Cao Xiao.
\newblock Fast{GCN}: Fast learning with graph convolutional networks via
  importance sampling.
\newblock In {\em Proc. of ICLR}, 2018.

\bibitem[\protect\citeauthoryear{DS \bgroup \em et al.\egroup
  }{2017}]{drugbank}
Wishart DS, Feunang YD, Guo AC, Lo~EJ, Marcu A, Grant JR, Sajed T, Li~C
  Johnson~D, Sayeeda Z, Assempour N, Iynkkaran I, Liu Y, Maciejewski A, Gale N,
  Wilson A, Chin L, Cummings R, Le~D, Pon A, Knox C, and Wilson M.
\newblock Drugbank 5.0: a major update to the drugbank database for 2018.
\newblock 2017.

\bibitem[\protect\citeauthoryear{Fey and Lenssen}{2019}]{fey2019fast}
Matthias Fey and Jan~Eric Lenssen.
\newblock Fast graph representation learning with pytorch geometric.
\newblock {\em arXiv preprint arXiv:1903.02428}, 2019.

\bibitem[\protect\citeauthoryear{Franceschi \bgroup \em et al.\egroup
  }{2019}]{franceschi2019-LearningDiscreteStrucutes}
Luca Franceschi, Mathias Niepert, Massimiliano Pontil, and Xiao He.
\newblock Learning discrete structures for graph neural networks.
\newblock In {\em Proc. of ICML}, 2019.

\bibitem[\protect\citeauthoryear{Gilmer \bgroup \em et al.\egroup
  }{2017}]{gilmer2017neural}
Justin Gilmer, Samuel~S Schoenholz, Patrick~F Riley, Oriol Vinyals, and
  George~E Dahl.
\newblock Neural message passing for quantum chemistry.
\newblock In {\em Proc. of ICML}, pages 1263--1272, 2017.

\bibitem[\protect\citeauthoryear{Hamilton \bgroup \em et al.\egroup
  }{2017}]{hamilton2017-GraphSAGE}
William Hamilton, Rex Ying, and Jure Leskovec.
\newblock Inductive representation learning on large graphs.
\newblock In {\em Proc. of NeurIPS}, 2017.

\bibitem[\protect\citeauthoryear{Huang \bgroup \em et al.\egroup
  }{2018}]{adaptive18}
Wenbing Huang, Tong Zhang, Yu~Rong, and Junzhou Huang.
\newblock Adaptive sampling towards fast graph representation learning.
\newblock In {\em Proc. of NeurIPS}, page 4563–4572, 2018.

\bibitem[\protect\citeauthoryear{Huang \bgroup \em et al.\egroup
  }{2019}]{caster19}
Kexin Huang, Cao Xiao, Trong~Nghia Hoang, Lucas~M. Glass, and Jimeng Sun.
\newblock {CASTER:} predicting drug interactions with chemical substructure
  representation.
\newblock {\em CoRR}, abs/1911.06446, 2019.

\bibitem[\protect\citeauthoryear{Kipf and Welling}{2017}]{kip2017-GCN}
Thomas Kipf and Max Welling.
\newblock Semi-supervised learning with graph convolutional neural networks.
\newblock In {\em Proc. of ICLR}, 2017.

\bibitem[\protect\citeauthoryear{Lu and Zhou}{2011}]{Lu2011LinkPI}
Linyuan Lu and Tao Zhou.
\newblock Link prediction in complex networks: A survey.
\newblock {\em ArXiv}, abs/1010.0725, 2011.

\bibitem[\protect\citeauthoryear{Ma \bgroup \em et al.\egroup
  }{2018}]{ma2018drug}
Tengfei Ma, Cao Xiao, Jiayu Zhou, and Fei Wang.
\newblock Drug similarity integration through attentive multi-view graph
  auto-encoders.
\newblock In {\em Proc. of IJCAI}, page 3477–3483, 2018.

\bibitem[\protect\citeauthoryear{Ma \bgroup \em et al.\egroup }{2019}]{genn19}
Tengfei Ma, Junyuan Shang, Cao Xiao, and Jimeng Sun.
\newblock {GENN:} predicting correlated drug-drug interactions with graph
  energy neural networks.
\newblock {\em CoRR}, abs/1910.02107, 2019.

\bibitem[\protect\citeauthoryear{Ryu \bgroup \em et al.\egroup
  }{2018}]{ryu2018deep}
Jae~Yong Ryu, Hyun~Uk Kim, and Sang~Yup Lee.
\newblock Deep learning improves prediction of drug--drug and drug--food
  interactions.
\newblock {\em Proc. of the National Academy of Sciences},
  115(18):E4304--E4311, 2018.

\bibitem[\protect\citeauthoryear{Schlichtkrull \bgroup \em et al.\egroup
  }{2018}]{schlichtkrull2018modeling}
Michael Schlichtkrull, Thomas~N Kipf, Peter Bloem, Rianne Van Den~Berg, Ivan
  Titov, and Max Welling.
\newblock Modeling relational data with graph convolutional networks.
\newblock In {\em Proc. of ESWC}, pages 593--607. Springer, 2018.

\bibitem[\protect\citeauthoryear{Shang \bgroup \em et al.\egroup
  }{2019}]{shang2019end}
Chao Shang, Yun Tang, Jing Huang, Jinbo Bi, Xiaodong He, and Bowen Zhou.
\newblock End-to-end structure-aware convolutional networks for knowledge base
  completion.
\newblock In {\em Proc. of AAAI}, pages 3060--3067, 2019.

\bibitem[\protect\citeauthoryear{Tatonetti \bgroup \em et al.\egroup
  }{2012}]{Tatonetti2012DatadrivenPO}
Nicholas~P. Tatonetti, Patrick Ye, Roxana Daneshjou, and Russ~B. Altman.
\newblock Data-driven prediction of drug effects and interactions.
\newblock {\em Science translational medicine}, 4 125:125ra31, 2012.

\bibitem[\protect\citeauthoryear{Vashishth \bgroup \em et al.\egroup
  }{2020}]{vashishth2020composition}
Shikhar Vashishth, Soumya Sanyal, Vikram Nitin, and Partha Talukdar.
\newblock Composition-based multi-relational graph convolutional networks.
\newblock {\em Proc. of ICLR}, 2020.

\bibitem[\protect\citeauthoryear{Vilar \bgroup \em et al.\egroup
  }{2014}]{ddisimilarity}
Santiago Vilar, Eugenio Uriarte, Lourdes Santana, Tal Lorberbaum, George
  Hripcsak, and Nicholas Tatonetti.
\newblock Similarity-based modeling in large-scale prediction of drug-drug
  interactions.
\newblock {\em Nature protocols}, 9:2147--2163, 09 2014.

\bibitem[\protect\citeauthoryear{Williams}{1992}]{reinforce}
Ronald~J. Williams.
\newblock Simple statistical gradient-following algorithms for connectionist
  reinforcement learning.
\newblock {\em Mach. Learn.}, 8(3–4):229–256, May 1992.

\bibitem[\protect\citeauthoryear{Xu \bgroup \em et al.\egroup
  }{2019}]{xu2019mrgnn}
Nuo Xu, Pinghui Wang, Long Chen, Jing Tao, and Junzhou Zhao.
\newblock {MR-GNN:} multi-resolution and dual graph neural network for
  predicting structured entity interactions.
\newblock {\em Proc. of IJCAI}, pages 3968--3974, 2019.

\bibitem[\protect\citeauthoryear{Xu \bgroup \em et al.\egroup
  }{2020}]{xu2020dynamically}
Xiaoran Xu, Wei Feng, Yunsheng Jiang, Xiaohui Xie, Zhiqing Sun, and Zhi-Hong
  Deng.
\newblock Dynamically pruned message passing networks for large-scale knowledge
  graph reasoning.
\newblock {\em Proc. of ICLR}, 2020.

\bibitem[\protect\citeauthoryear{Yang \bgroup \em et al.\egroup
  }{2015}]{yang2014embedding}
Bishan Yang, Wen{-}tau Yih, Xiaodong He, Jianfeng Gao, and Li~Deng.
\newblock Embedding entities and relations for learning and inference in
  knowledge bases.
\newblock {\em Proc. of ICLR}, 2015.

\bibitem[\protect\citeauthoryear{Ying \bgroup \em et al.\egroup
  }{2018}]{ying2018graph}
Rex Ying, Ruining He, Kaifeng Chen, Pong Eksombatchai, William~L Hamilton, and
  Jure Leskovec.
\newblock Graph convolutional neural networks for web-scale recommender
  systems.
\newblock In {\em Proc. of KDD}, pages 974--983, 2018.

\bibitem[\protect\citeauthoryear{Zeng \bgroup \em et al.\egroup
  }{2020}]{zeng2020graphsaint}
Hanqing Zeng, Hongkuan Zhou, Ajitesh Srivastava, Rajgopal Kannan, and Viktor
  Prasanna.
\newblock Graphsaint: Graph sampling based inductive learning method.
\newblock {\em Proc. of ICLR}, 2020.

\bibitem[\protect\citeauthoryear{Zitnik \bgroup \em et al.\egroup
  }{2018}]{zitnik2018modeling}
Marinka Zitnik, Monica Agrawal, and Jure Leskovec.
\newblock Modeling polypharmacy side effects with graph convolutional networks.
\newblock {\em Bioinformatics}, 34(13):i457--i466, 2018.

\end{thebibliography}


==> sec/approach1_backup.tex <==
\section{Modeling Edge-Type Probabilities} % for Neighborhood Sampling}
\label{sec:approach1}
Graph neural networks have proven successful in various tasks, such as for link prediction, and they have been successfully extended to multi-relational graphs. However, the computational complexity of these models is too high for very large graphs. Motivated by the solutions in homogeneous graphs, we propose a new sampling technique tailored to multi-relational graphs, based on probabilities for edge types. %Specifically, we incorporate a probability for each edge type into the reasoning process over multi-relational graphs. We propose a new {relation-dependent sampling based graph convolutional networks}. %, called {\ourmodel}. 

\subsection{Relation Sampling in Multi-Relational Message Passing}
\label{sec:modelone}
In some previous sampling approaches for GCNs~\cite{chen2018fastgcn,adaptive18}, the message-passing schema of GCN is rewritten to an expectation form over the prior distribution of all nodes. Reconsidering the formulation of R-GCN \eqref{eq:rgcn}, we can similarly reformulate it into an expectation form. However, instead of using the node distribution, we rather focus on the distribution of relations. When $c_{u,r}=\frac{1}{|\mathcal{N}_{u,r}|}$, the R-GCN Equation (\ref{eq:rgcn}) can be rewritten in the following expectation form.
\begin{align}
     h_u^{l+1} & = & \phi \left( W_0^l h_u^l  + |\mathcal{R}| \mathbb{E}_{p(r|u)} \mathbb{E}_{p(v|u,r)}( W_r^l h_v^l) \right) \notag\\
     & = & \phi \left( W_0^l h_u^l  + |\mathcal{R}| \mathbb{E}_{p(r,v|u)} ( W_r^l h_v^l) \right)\label{eq:expectation}
\end{align}
where  $p(r|u) = \frac{1}{|\mathcal{R}|}$ defines the probability of relation type $r$ conditioned on the node $u$ ($|\mathcal{R}|$ is the number of relation types, and the probability for each $r$ is the same); $p(v|u,r) = c_{u,r} = \frac{1}{|\mathcal{N}_{u,r}|}$ indicates a uniform distribution of neighbor nodes connecting to $u$ through relation $r$; and $p(r,v|u) = p(r|u)p(v|u,r)$ indicates the joint distribution of $r$ and $v$ given $u$, i.e., the probability of an edge $(u,r,v)$. 

To speed up message passing in a large, dense graph with many different relation types, a natural solution is to approximate the expectation component in Equation~\eqref{eq:expectation} by Monte Carlo sampling. For each node $u$, we can sample a set of $m$ edges in its neighborhood, approximating Equation~\eqref{eq:expectation}:
\begin{equation}
    h_u^{l+1} \simeq \phi \left( W_0^l h_u^l + \frac{|\mathcal{R}|}{m} \sum_{r,v \sim p(r,v|u)}  W_r^l h_v^l\right)
    \label{eq:rgcn_sampling}
\end{equation}

% distribution of relations:
% \begin{equation}
%      h_u^{l+1} = \phi \left( W_0^l h_u^l  + \mathbb{E}_{p(r|u)}( \sum_{v\in\mathcal{N}_{u,r}} W_r^l h_v^l) \right)
%      \label{eq:expectation}
% \end{equation}
% where $p(r|u) = \frac{c_{r,u}}{\sum_r c_{r,u}}$ defines the probability of relation $r$ conditioned on the node $u$.

% To speed up message passing in a large dense graph with many different relation types, one solution is to approximate the expectation component in Equation~\eqref{eq:expectation} by Monte Carlo sampling. For each node $u$, we can sample a small number $m$ of relations in its neighborhood, and Equation~\eqref{eq:expectation} is approximated by:
% \begin{equation}
%     h_u^{l+1} \simeq \phi \left( W_0^l h_u^l + \frac{1}{m} \sum_{r \sim p(r|u)} \sum_{v\in\mathcal{N}_{u,r}} W_r^l h_v^l\right)
%     \label{eq:inverse_sampling}
% \end{equation}


% \subsection{Extending Message Passing}
% \label{sec:probemb}
% A very straightforward idea to incorporate edge-type importance into R-GCNs is to extend Equation~\eqref{eq:rgcn} by modeling the importance assigned to each edge type based on the local neighborhood. 
% That is, we consider an additional learnable parameter $l_r$ for each edge type $r\in\mathcal{R}$.
% During node update, we then calculate a softmax distribution based on the local neighborhood and the new parameters as follows:
% \begin{align*}
% c_{u,r} &= \frac{e^{l_{r}}}{\sum_{r'\in\mathcal{R}} {|\mathcal{N}_{u,r'}|} e^{l_{r'}}}
% \end{align*}
% Note that, while related works using R-GCN usually apply a simple factor like $c_{u,r} = \frac{1}{|\mathcal{N}_{u,r}|}$ as suggested in \cite{kip2017-GCN}, the latter mention that $c_{u,r}$ might be learned as well. Here, we try to achieve that by defining $c_{u,r}$ in terms of learnable parameters $l_r$ and interpreting it as the probability, or importance, assigned to edge type $r$ by node $u$.
% % Observe that we can consider $\alpha_{u,r}$ as a part of $c_{u,r}$. Indeed, while related works using R-GCN usually apply a simple factor like $c_{u,r} = \frac{1}{|\mathcal{N}_{u,r}|}$ as suggested in \cite{kip2017-GCN}, the latter mention that $c_{u,r}$ might be learned as well. Hence, we here consider $c_{u,r} = \frac{1}{|\mathcal{N}_{u,r}|} * \alpha_{u,r}$.
% %Also note that a similar edge-weight parameter has been included into GCNs in \cite{shang2019end}, but their goal was 
% % 
% Probabilities integrated in this way during the message passing stage offer a certain level of explainability, but no solution in terms of scalability. Therefore we alternatively study incorporating them in the sampling stage.

\subsection{\ourmodel: Relation Sampling based on Learned Probabilities}
\label{sec:probsampling}
In the R-GCN model, each relation type $r$ has the same weight %or probability 
in the aggregation function. However, we argue that the relation types matter and propose to learn their weights automatically. Different relation types occur with different frequency and have different semantics. These factors should largely impact the importance of relations, hence we posit that modeling relation-dependent probabilities is beneficial.
%denotes the set of nodes connected to node $u$.

A straightforward idea to incorporate edge-type importance into R-GCN is to extend Equation~\eqref{eq:rgcn} by regarding $c_{u,r}$ as a learnable, normalized parameter. That is, we consider an additional, learnable parameter $l_r$ for each edge type $r\in\mathcal{R}$, and define the weight for each neighborhood as follows:
\begin{align*}
c_{u,r} &= \frac{e^{l_{r}}}{\sum_{r'\in\mathcal{R}} {|\mathcal{N}_{u,r'}|} e^{l_{r'}}}
\end{align*}
We call this variant \textbf{relation-weighted GCN (\ourmodelone)}.

Since our goal is scalability, we further consider sampling. As outlined in Figure~\ref{fig:sampling_process},
% More specifically,
% based on the new parameters and define our \textbf{relation-dependent sampling-based graph convolutional  network (RS-GCN)}:
% \begin{equation}
%     h_u^{l+1} \simeq \phi \left( W_0^l h_u^l + \frac{1}{m} \sum_{r,v \sim p(r,v|u)}  W_r^l h_v^l\right)
%     \label{eq:rs-gcn_sampling}
% \end{equation}
% where $p(r,v|u) = c_{u,r}$ and $m$ is the number of samples. We then can take this learnable relation-specific probability and 
we can incorporate a uniform probability $p(r,v|u)$ %(in the figure, we have $p_{r,k}$) 
into a neighborhood sampling schema similar to GraphSAGE \cite{hamilton2017-GraphSAGE}. %$As shown in Figure~\ref{fig:sampling_process}, f

For each target edge (prediction), we sample a fixed-sized $k$-hop neighborhood for both nodes in it iteratively (i.e., for $k=1,2,\dots$), and then perform message passing using Equation~\eqref{eq:rgcn}. 
% Specifically, we use the edge-type parameters $l_r$ to generate a softmax distribution over all the edges in that hop and sample $n_k = s_k * |\mathcal{N}_{k-1}|$ edges from it with replacement; here $s_k$ is the number of edges to sample in hop $k$ for each node in hop $k-1$, $\mathcal{N}_{k-1}$ is the set of nodes sampled in hop $k-1$.
%(~\ref{eq:rgcn_sampling}). 
The main difference to GraphSAGE is that our method samples relations, not nodes. The uniform sampling drives the updating schema for \ourmodelone as:
\begin{equation}
    h_u^{l+1} \simeq \phi \left( W_0^l h_u^l + \frac{1}{m} \sum_{r,v \sim p(r,v|u)}  c_{u,r} W_r^l h_v^l\right)
    \label{eq:rs-gcn_sampling}
\end{equation}
where $m$ is the number of samples, $p(r,v|u) = 1/|\mathcal{N}_u|$ and $\mathcal{N}_u = \cup_r \mathcal{N}_{u,r}$
\mathcal{u}
% However, if we use uniform sampling in Equation~\eqref{eq:rgcn_sampling}, we do not really model edge-type \emph{probabilities} since the factor $|\mathcal{R}|$ obtained from R-GCN in Equation~\eqref{eq:rgcn} yields that the values do not necessarily sum up to $1$.
%Note that this sampling scheme is independent of edge types. A better strategy is to also consider the importance of edge types in the sampling phase. 
However, uniform sampling is inefficient for it still ignores the importance of the edge types in the sampling schema. We therefore consider a slightly adapted importance sampling version
\begin{equation}
    h_u^{l+1} \simeq \phi \left( W_0^l h_u^l + \frac{1}{m} \sum_{r,v \sim p(r,v|u)}  W_r^l h_v^l\right)
    \label{eq:rs-gcn_sampling}
\end{equation}
where $p(r,v|u) = c_{u,r}$ is a not uniform but a learnable parameter.

Specifically, based on Equation (\ref{eq:rs-gcn_sampling}) we propose the \textbf{relation-dependent sampling-based graph convolutional network (RS-GCN)}, which \emph{learns} sampling probabilities for each edge type during training instead of using uniform sampling as above and in GraphSAGE. The idea is to learn how to retain a useful neighborhood around an edge without compromising scalability, while tightly coupling message passing and sampling through the parameters. Similar to \ourmodelone, \ourmodel uses latent parameters $l_r$; they are initialized with elements $l_r \sim \mathcal{N}(0, 1)$. 
%For a given target edge, we sample a fixed-sized $k^{th}$-hop neighborhood around that edge iteratively (i.e., for $k=1,2,\dots$) to obtain a subgraph. 
In practice, following GraphSAGE we only sample two hops. In each hop $k$ during sampling, we use the edge-type parameters $l_r$ to generate a distribution over all the edges in that hop and sample $n_k = s_k * |\mathcal{N}_{k-1}|$ edges from it with replacement; here $s_k$ is the number of edges to sample in hop $k$ for each node in hop $k-1$, $\mathcal{N}_{k-1}$ is the set of nodes sampled in hop $k-1$. 
The sampling probability for an edge with type $r$ in the $k$-th hop is defined as: 
\begin{align*}
    p_{r,k} &= \frac{e^{l_{r}}}{\sum_{r'\in\mathcal{R}} {|\mathcal{E}_{k,r'}|} e^{l_{r'}}}
\end{align*}
where $\mathcal{E}_{k,r'}$ is the set of edges of relation type $r'$ in hop $k$.
This $p_{r,k}$ is exactly the $p(r,v|u)$ in Equation~\ref{eq:rs-gcn_sampling}. \ourmodel thus is actually an R-GCN variant parameterizing $p_{r,k}$ instead of $c_{u,r}$ in Equation~\eqref{eq:rgcn}. We will use this kind of sampling in combination with R-GCN and RW-GCN in our evaluation. 

% TBD!!! which k for $c_ur$? the final one?
% $\mathcal{N}_{k-1}$ is the set of nodes sampled in hop $k-1$. The sampling probability for an edge type $r$ in the $k$-th hop can be calculated as follows: 
% \begin{align*}
%     p_{r,k} &= \frac{e^{l_{r}}}{\sum_{r'\in\mathcal{R}} {|\mathcal{N}_{k,r'}|} e^{l_{r'}}}
% \end{align*}
% where $\mathcal{N}_{k,r'}$ is the set of edges in hop $k$ with relation type $r'$.

% For each of the two nodes in a given node pair, we then sample a $k$-hop neighborhood iteratively (i.e., for $k=1,2,\dots$) by selecting a neighbor connected through edge type $r$ with the corresponding learned probability.
% This effectively makes the sampling adapt to the frequency and importance of edge types in the problem. Our evaluation later shows what this means for different example datasets. 
% More scalable 2. Indicates how long an edge type can pass messages
\subsection{Learning Relation Probabilities}
As there are difficulties in backpropagating through the sampled subgraph, we use the score function estimator REINFORCE \cite{reinforce}. For a loss function $L$ and sampled subgraph $g$, to estimate the gradient of the loss with respect to the latent parameters $l=(l_0,\dots,l_{|\mathcal{R}|})$, we compute $p_l(g)$, the probability of sampling $g$ given $l$:
\begin{align*}
    \nabla_{l} \mathop{{}\mathbb{E}_g} [L(g)] = \mathop{{}\mathbb{E}_g} [L(g) \nabla_{l} \log p_{l}(g)]
\end{align*}
In this way, REINFORCE does not require backpropagation through the message passing layers or the sampled subgraph if we can compute $\nabla_{l} \log p_{l}(g)$. We observe that this can be achieved easily by computing $\log p_{l}(g)$ as below and backpropagating the gradient; $r_i$ is the edge type of the $i^{th}$ edge sample: 
\begin{align*}
   \log p_{l}(g) &= \sum_{k} \sum_{i=1}^{n_k} \log p_{r_i,k} \\&
                 = \sum_{k} \sum_{i=1}^{n_k} \log {\frac{e^{l_{r_i}}}{\sum_{r'\in\mathcal{R}} {|\mathcal{E}_{k,r'}|} e^{l_{r'}}}}
\end{align*}
Note that REINFORCE gives an unbiased estimator but may incur high variance. The variance can be reduced by using control variate based variants of REINFORCE which is left as future work.

\paragraph{Discussion} Learning edge probabilities has been explored in different contexts. \cite{adaptive18} proposed a neural network to learn the optimum probability for importance sampling of the nodes in each layer. However, they focus on approximation of the homogeneous GCN model and their objective for optimum sampling is to reduce the variance. \cite{franceschi2019-LearningDiscreteStrucutes} incorporate a Bernoulli distribution for sampling the latent graph structures and, at the same time, automatically learn the hyperparameters of the distribution. In our case the graph structure is already given and our edge probability is assigned to known edges. Moreover, our sampling method is different form importance sampling~\cite{chen2018fastgcn}. For importance sampling, we have the fixed prior $p(r,v|u)$ and use another sampling probability $q(r,v)$ to approximate the expectation; but in our model we directly make $p(r,v|u)$ learnable and infer it from the model.

% Second, we consider Gumbel-Softmax \cite{jang2017-gumbelsoftmax}, a method that allows to obtain a  differentiable sample from a discrete distribution. Hence, our sampling becomes differentiable and the edge-type probabilities can be learned directly. Gumbel-softmax reduces variance at the cost of having biased estimates of gradients. 

% When the graph $G$ is input to the model, we compute the sampling logits $Ap$. Based on these logits, we use Gumbel-Softmax to sample from the $k$-hop neighborhood of each target edge \cite{jang2017-gumbelsoftmax}. The Gumbel-Softmax ``straight-through trick" allows this sampling to be differentiable, so the edge parameters can be learned directly. Due to some technical constraints with PyTorch Geometric's RGCN implementation \cite{Fey/Lenssen/2019}, we also implement this learnable sampling using a score function estimator, known as REINFORCE \cite{reinforce}. It treats the outer objective as a black box function and does not require differentiability with respect to sampling parameters. REINFORCE gives an unbiased estimator but usually has high variance. On the other hand, Gumbel-softmax reduces variance at the cost of having biased estimates of gradients. 






==> sec/approach2.tex <==
\section{Additional Evidence for DDI Prediction: Drug Mixtures and Synergies} 
\label{sec:approach2}

Past research has shown that random negative sampling and including various types of data (e.g., drug-protein interactions) help to improve DDI prediction \cite{zitnik2018modeling}. 
%
We propose to apply compound pairs contained in marketed drug mixture products, available from \drugbank \cite{drugbank}, and knowledge about drugs that synergize, available from \drugcombdb \cite{drugcombdb}. For side effect prediction, this data can be considered as verified negative evidence (vs. random, possibly incorrect negative samples). For general DDI prediction, it can provide signals towards positive DDI types. To the best of our knowledge, this has not been studied before. For simplicity, we will call all this data synergistic evidence in the following (i.e., although the compounds from mixtures do not necessarily yield synergistic effects, which means effects that are higher than if the drugs are taken individually).

To incorporate that evidence into our model, we propose two approaches. 
For side effect prediction, we use it as negative samples during the computation of the loss function (i.e., during training and validation). While we thus include a more reliable set of negative samples, the extra information is not incorporated into the model yet.
%
Therefore, we also consider the synergistic evidence as a new edge type in the graph data to allow GNNs to use the extra information when computing node embeddings. 





==> sec/stmt.tex <==
\newpage
\section*{Statement of Broader Impact}

Graph data has a pervasive impact in many diverse fields and the popularity of graph neural networks certainly increases the danger of an application with negative effects (even if just due to ignorance).
As pointed out in this work w.r.t.\ negative sampling, we have to be aware of the risks of standard AI techniques, and should always evaluate if and how they can be applied to the problem at hand.

Nevertheless, the variety of applications also yields broad inspiration for the development of new graph neural networks. Many of the basic graph neural network architectures have been influenced by specific applications (e.g., message-passing neural networks by quantum chemistry \cite{gilmer2017neural}).

Personally, we believe that biomedicine is one of the application areas where our graph neural networks provide the greatest benefits, for both the current society and future generations.
Our research has centered on problems and datasets as the ones studied in this paper for some time [citations removed for anonymity], and we hope that our papers motivate other researchers to target similar applications.

\section*{Acknowledgements} 
[removed for anonymity]
% \veronika{Rico do you have some grant or similar?}
\section*{Funding Disclosures}
[removed for anonymity]
